MOA-2020-BLG-135Lb: A New Neptune-class Planet for the Extended MOA-II Exoplanet Microlens Statistical Analysis

We report the light-curve analysis for the event MOA-2020-BLG-135, which leads to the discovery of a new Neptune-class planet, MOA-2020-BLG-135Lb. With a derived mass ratio of $q=1.52_{-0.31}^{+0.39} \times 10^{-4}$ and separation $s\approx1$, the planet lies exactly at the break and likely peak of the exoplanet mass-ratio function derived by the MOA collaboration (Suzuki et al. 2016). We estimate the properties of the lens system based on a Galactic model and considering two different Bayesian priors: one assuming that all stars have an equal planet-hosting probability and the other that planets are more likely to orbit more massive stars. With a uniform host mass prior, we predict that the lens system is likely to be a planet of mass $m_\mathrm{planet}=11.3_{-6.9}^{+19.2} M_\oplus$ and a host star of mass $M_\mathrm{host}=0.23_{-0.14}^{+0.39} M_\odot$, located at a distance $D_L=7.9_{-1.0}^{+1.0}\;\mathrm{kpc}$. With a prior that holds that planet occurrence scales in proportion to the host star mass, the estimated lens system properties are $m_\mathrm{planet}=25_{-15}^{+22} M_\oplus$, $M_\mathrm{host}=0.53_{-0.32}^{+0.42} M_\odot$, and $D_L=8.3_{-1.0}^{+0.9}\; \mathrm{kpc}$. This planet qualifies for inclusion in the extended MOA-II exoplanet microlens sample.

==> aastex63_additional_journal_abbreviations.tex <==
\newcommand\cse{\ref@jnl{CSE}}%     %  Computing In Science Engineering %%CR Added

